LoRE-Merging: Exploring Low-Rank Estimation For Large Language Model Merging

While most current approaches rely on further training techniques, such as fine-tuning or reinforcement learning, to enhance model capacities, model merging stands out for its ability of improving models without requiring any additional training. In this paper, we propose a unified framework for model merging based on low-rank estimation of task vectors without the need for access to the base model, named \textsc{LoRE-Merging}. Our approach is motivated by the observation that task vectors from fine-tuned models frequently exhibit a limited number of dominant singular values, making low-rank estimations less prone to interference. We implement the method by formulating the merging problem as an optimization problem. Extensive empirical experiments demonstrate the effectiveness of our framework in mitigating interference and preserving task-specific information, thereby advancing the state-of-the-art performance in model merging techniques.

==> src/response.tex <==
Response & revisions
We sincerely appreciate the valuable feedback provided by the reviewers in the ACL ARR February cycle and extend our gratitude to the meta-reviewer and reviewers for their constructive comments. For the new submission, we have made substantial revisions to address their suggestions and enhance the overall quality of our work. As the main concerns have been included in the meta-reviews, we provide a point-by-point response to the weakness mentioned in meta-review. 

Response to Meta-review
Q1: The claim that LORE-MERGING does not require access to the base model seems irrelevant in real-world scenarios, as typically, base model access is available and important for model merging tasks.

A1: Firstly, from a theoretical perspective, this assumption aligns with the prior work, notably like Fisher Merging[1]. While our theoretical foundation builds upon these works, our empirical motivation stems primarily from checkpoint merging phenomena as presented in Liu et al. [2]. In the context of checkpoint merging, it is hard to assign or identify a base model, as the constituent checkpoints perform comparably with equivalent status in the merging hierarchy. In real applications, for example, we would like to merge DeepSeekMath and Numina-Math, none of them can be assigned as the base model since both models are fully fine-tuned versions.

[1] Matena M S, Raffel C A. Merging models with fisher-weighted averaging[J]. Advances in Neural Information Processing Systems, 2022, 35: 17703-17716.
[2] Liu D, Wang Z, Wang B, et al. Checkpoint merging via bayesian optimization in llm pretraining[J]. arXiv preprint arXiv:2403.19390, 2024.

Q2: The approach relies on a straightforward low-rank optimization technique, but lacks deeper theoretical grounding or explanation on why it outperforms existing methods, such as Ties-Merging and DARE.

A2: Our low-rank assumption derives from the theoretical underpinnings of the LoRA, which posits that specialized capabilities within LLM can be effectively parameterized via low-rank matrix representations. Through extensive empirical validation, we have observed that task vectors consistently exhibit low-rank properties across various domains. This fundamental observation constitutes the primary theoretical foundation of our research.

We also offer potential explanations for why LoRE-Merging outperforms existing methods such as Ties-Merging and DARE. Regarding DARE, we identify two possible reasons: (1) As noted in the original DARE study, it is more suitable for merging models with smaller parameter discrepancies. However, WizardLM and WizardMath are domain-specific models with substantial parameter differences. Based on this assumption, DARE performs well in scenarios involving checkpoint merging where the differences between checkpoints are minimal. (2) DARE randomly discards certain parameters of task vectors, which may result in the loss of crucial task-specific features due to the randomness of this approach. For Ties-Merging, similar to DARE, it also discards some vectors, retaining only those with the highest magnitudes. This selective preservation can similarly lead to the omission of important features.

Q3: There is insufficient evidence to prove its generalization ability in more diverse multi-task settings, like code-related reasoning tasks.

A3: It is a good suggestion. We have supplied results on new benchmarks, including MMLU, GLUE and MBPP.

Key Revisions:
We have made substantial revisions to address their suggestions and enhance the overall quality of our work. The key revisions are summarized as following:
1. We improve the writing quality according to the suggestions from last round.
2. We provide new evaluation results on more benchmarks, like MMLU, GLUE and MBPP datasets.
3. Ablation study on hyper-parameters are provided in the new version.
4. We elaborate the computational overhead and the efficiency of LoRE-Merging.

